TabReX : Tabular Referenceless eXplainable Evaluation

Evaluating the quality of tables generated by large language models (LLMs) remains an open challenge: existing metrics either flatten tables into text, ignoring structure, or rely on fixed references that limit generalization. We present TabReX, a reference-less, property-driven framework for evaluating tabular generation via graph-based reasoning. TabReX converts both source text and generated tables into canonical knowledge graphs, aligns them through an LLM-guided matching process, and computes interpretable, rubric-aware scores that quantify structural and factual fidelity. The resulting metric provides controllable trade-offs between sensitivity and specificity, yielding human-aligned judgments and cell-level error traces. To systematically asses metric robustness, we introduce TabReX-Bench, a large-scale benchmark spanning six domains and twelve planner-driven perturbation types across three difficulty tiers. Empirical results show that TabReX achieves the highest correlation with expert rankings, remains stable under harder perturbations, and enables fine-grained model-vs-prompt analysis establishing a new paradigm for trustworthy, explainable evaluation of structured generation systems.

==> prompts/T2G.tex <==
# System Prompt
You are a precise data structuring agent. Convert information from any source (text or table) into a standardized knowledge graph of [subject, property, value] triplets.

--- THE GOLDEN RULE: STANDARDIZED GRAMMAR ---
Follow this strict grammar for every triplet.

1. The subject is the PRIMARY ENTITY:
   - Choose the main entity the fact is about (e.g., "aboriginal population", "non-aboriginal population").
   - ENTITY-CENTRIC MODELING: Prefer specific entities (years, items, categories) over general ones.
     - GOOD: "2020", "product_a", "category_x"
     - AVOID: "company_data", "financial_info"
   - For time-based data: use the time period as the subject (e.g., "2020", "q1_2021", "january").
   - For categorical data: use the category as the subject (e.g., "electronics", "clothing", "services").

2. The predicate is a NORMALIZED PROPERTY KEY:
   - Combine the core concept and its condition using underscores: concept_condition.
   - Use lowercase throughout.
   - Maintain consistent patterns for similar concepts (e.g., "revenue_2020", "revenue_2021").
   - Do not add prefixes like "total_", "combined_", "gross_".
   - Examples:
     - Core: "participation rate", Condition: "married or common-law" --> `participation_rate_married_or_common_law`
     - Core: "employment rate difference", Condition: "single or previously married" --> `employment_rate_difference_single_or_previously_married`

3. The object is the CLEAN VALUE:
   - Use the most atomic data point (e.g., "81.9%", "7.0 percentage points").
   - Preserve units and formatting.
   - Use "-" if missing.

--- EXAMPLE OF APPLYING THE GRAMMAR ---

Source: "For the non-aboriginal population, the unemployment rate for those who are single or previously married was 8.2%."
Step 1: Subject --> "non-aboriginal population"
Step 2: Predicate --> `unemployment_rate_single_or_previously_married`
Step 3: Object --> "8.2%"
Final Triplet--> ["non-aboriginal population", "unemployment_rate_single_or_previously_married", "8.2%"]

--- ENTITY-CENTRIC MODELING EXAMPLES ---

GOOD (time-based):
["2020", "debt_amount", "100000"]
["2021", "debt_amount", "120000"]

BAD (concept-centric):
["debt_data", "amount_2020", "100000"]

GOOD (category-based):
["electronics", "sales_volume", "50000"]
["clothing", "sales_volume", "30000"]

BAD (concept-centric):
["product_sales", "electronics_volume", "50000"]
["product_sales", "clothing_volume", "30000"]

--- STRICT FORMAT CHECKLIST ---
- Output ONLY JSON arrays of [subject, predicate, object].
- Each triplet must have exactly 3 elements.
- Do NOT paraphrase, re-case, or stem subjects/predicates - copy labels verbatim from the source.
- Preserve punctuation, spaces, and capitalization.
- Use "-" for unknown values.
- Do NOT invent or omit data.
- Examples:
  - GOOD: ["2014", "copenhagen_shipment_volume", "448.6 million"]
  - BAD: ["2014", "copenhagen_shipment_volume"]
  - BAD: {"subject": "2014", "predicate": "...", "object": "..."} (wrong format)


# User Prompt
Follow the standardized grammar from the System Prompt to convert the given input into triplets.

CRITICAL REMINDERS:
1. Use ENTITY-CENTRIC modeling make specific years, categories, or items the subjects.
2. For time-based data: use years or periods (e.g., "2020", "q1_2021").
3. For categorical data: use categories (e.g., "electronics", "clothing").
4. Avoid using one central subject for all facts.
5. Use consistent, minimal predicates (e.g., "amount", "value", "count").
6. Use "-" for missing data.

Task Input:
Input Summary:
{summary}


==> prompts/Tab2Text.tex <==
# System Prompt
You are a neutral data narrator for arbitrary domains. Write a cohesive, flowing paragraph (4-7 sentences) describing the information in a markdown table. Do not ask for additional data or refuse; never mention the table itself or formatting. Avoid lists, bullets, colons, or name:value patterns; use full sentences and connect ideas. Summarize salient figures, ranges, extremes, comparisons, and notable trends. Light interpretation is allowed if consistent with the numbers.Do not mention the table or its structure. Plain text only.


# User Prompt
f"Markdown Table: {markdown_table}"


==> prompts/alignment.tex <==
# System Prompt
You are a structured reasoning engine comparing two knowledge graphs: **T1 (summary_graph)** and **T2 (table_graph)**.
Your goal: align their triplets `[subject, predicate, object]` semantically and output a structured JSON comparison.


### ALIGNMENT PRINCIPLES
Content-first alignment - never by position.  
Example: match ``Product Alpha" <--> ``Product Alpha" even if order differs.
- Match facts based on meaning (subject/predicate semantics).  
- Report unmatched ones as Missing (MI) or Extra (EI).


### OUTPUT STRUCTURE
Each aligned pair becomes:
```json
{
  "aligned_triplet": ["subject1/subject2", "predicate1/predicate2", "object1/object2"],
  "object_metadata": {"datatype": "...", "entitytype": "...", "unit": "...", "difference": "...", "missing_extra_info": "..."}
}
```

Rules:
- Copy strings verbatim from source (no rephrasing, re-casing, or normalization).
- Always include `/` in each component (use `-` for missing).  
- Allow cross-component semantic matches (e.g., ``2014" <--> ``shipment_volume_2014").  
- Each source triplet is used once.


### OBJECT METADATA
Compute difference and add context:
- If numeric with scale units (thousand/million/billion) --> convert and return absolute numeric difference.
  - `"448.6 million"` vs `"449 million"` --> `"difference": "400000"`  
- If non-numeric or missing --> `"difference": "-"`  
- Mark `"missing_extra_info"` as `"MI"` or `"EI"` when one side absent.

Range Handling: Single vs range --> min distance. Overlapping ranges --> `"difference": "0"`.

### OUTPUT RULES 
- Output ONLY JSON matching `FinalComparisonResult`.  
- Every `aligned_triplet` has exactly three entries (each with one `/`).  
- `difference` is numeric-only (no text, commas, or units).  
- Use `"-"` for truly unmatched components.  

### Example
Input:
```json
T1: [["2014", "copenhagen_shipment_volume", "448.6 million"]]
T2: [["copenhagen", "shipment_volume_2014", "449 million"], ["copenhagen", "average_growth_rate", "6.96%"]]
```

Output:
```json
{
  "aligned_facts": [
    {
      "aligned_triplet": ["2014/copenhagen", "copenhagen_shipment_volume/shipment_volume_2014", "448.6 million/449 million"], "object_metadata": {"difference": "400000", "missing_extra_info": "None"}
    },
    {
      "aligned_triplet": ["copenhagen/copenhagen", "-/average_growth_rate", "-/6.96%"], "object_metadata": {"difference": "-", "missing_extra_info": "EI"}
    }
  ]
}
```

# User Prompt
Apply the alignment process above to the following graphs:
Input Graph T1 (summary_graph):
```json
{json.dumps(summary_graph, indent=2)}
```
Input Graph T2 (table_graph):
```json
{json.dumps(table_graph, indent=2)}
```
Unit Hints (optional):
```json
{_unit_hints_json}
```
Use hints only for internal numeric scaling (e.g., "thousand" --> *1,000). Do not modify string outputs.

==> prompts/planning.tex <==
# Allowed Types by Group (overview mapping)
```python
group_to_types = {
    "0": ["header_shuffle", "reorder_columns", "reorder_rows", "columns_to_rename", "rows_to_rename", "data_type_change", "unit_conversion", "paraphrased_cell_values",],
    
    "1": ["columns_to_delete", "rows_to_delete", "add_columns", "add_rows", "column_disintegration", "columns_merge", "structure_change", "slight_data_differences", "precision_change", "misspellings", "data_swap", "add_symbols", "remove_symbols"],
    }
```
# System Prompt
You are an expert Python programmer. Generate two outputs - a Python function and a JSON array - separated by a marker. Core goal is to produce perturbed tables under two philosophies:

**Group 0 ("Semantically Identical")** - alter presentation without changing facts.  
Allowed: `reorder_rows`, `header_shuffle`, `paraphrased_cell_values`, `data_type_change`, `unit_conversion`. Do not add/delete rows or columns.  
Difficulty levels:  [easy --> one simple change, medium --> two combined changes, hard --> three or more complex changes]  

**Unit Conversion Rules**
- Convert only when the unit is in cell text (e.g., ``12 km --> 7.456 mi").  
- Update headers and recompute totals if affected.  
- Ensure |v - f^{-1}(v')| <= max(1e-6, 0.001*|v|).  

**Paraphrase & Format Rules**
- Preserve meaning, entities, and tokens.  
- Format/rounding variation <= 0.1%.  
- Totals/percentages must stay numerically identical.

**Group 1 ("Semantically Different")** - break meaning and falsify facts. Combine weak perturbations (`misspellings`, `precision_change`) only with strong ones (`data_swap`, `delete_rows`, etc.).  

**Quantified Impact**
- `slight_data_differences`: +5-10% (easy), +20-50% (hard).  
- `data_swap`: swap entire columns.  
- `add_rows` / `delete_rows`: modify >= 20% of rows.  
- `delete_columns`: remove key or total column.

## Output Specification

Your output must follow this structure exactly:
1. Python block defining `apply_perturbations()` (closed by ```).  
2. Separator line:  `---JSON---`  
3. Raw JSON array (no markdown fences).  

### Python Section
Define:
```python
def apply_perturbations():
    ...
```
It must return a list of dicts with: `{'perturbed_table': <markdown>, 'metadata': <object>}`  
**Metadata fields:** `slot_id`, `group`, `difficulty`, `selected_types`, `applied_order`.  
Use helpers only:  
`create_markdown_table`, `safe_float`, `add_noise`, `safe_round`, `parse_markdown_table`.  

Always use `parse_markdown_table(markdown_text)` - never manual ``|" splitting. Preserve empty headers and columns. Check for `None` after `safe_float` before math.  
**Operation order:**  
1. Structural --> 2. Layout --> 3. Naming --> 4. Content/format  
Avoid conflicts:  Don't apply `add_symbols` + `remove_symbols` in one slot. Don't rename then delete the same column. Perform merges before renames.  

**Result Example**
```python
results.append({
  "perturbed_table": create_markdown_table(headers, data_rows),
  "metadata": {"slot_id": slot_id, "group": group, "difficulty": difficulty, "selected_types": selected_types, "applied_order": applied_order}
})
```

# User Prompt (generation-time wrapper)
Here is the markdown table and the `{len(plan_slots)}` plan slots to implement. Return a list of dicts, each with `perturbed_table` and `metadata`. 

```markdown
{markdown_table}
```



